SimAug: Learning Robust Representations from Simulation for Trajectory Prediction

This paper studies the problem of predicting future trajectories of people in unseen cameras of novel scenarios and views. We approach this problem through the real-data-free setting in which the model is trained only on 3D simulation data and applied out-of-the-box to a wide variety of real cameras. We propose a novel approach to learn robust representation through augmenting the simulation training data such that the representation can better generalize to unseen real-world test data. The key idea is to mix the feature of the hardest camera view with the adversarial feature of the original view. We refer to our method as SimAug. We show that SimAug achieves promising results on three real-world benchmarks using zero real training data, and state-of-the-art performance in the Stanford Drone and the VIRAT/ActEV dataset when using in-domain training data.

==> tables/actev.tex <==
\begin{table}[]

\centering
\caption{State-of-the-art comparison on the VIRAT/ActEV dataset. Numbers are minimal errors over 1 predictions and lower the better. %The methods marked by $\star$ use real VIRAT/ActEV training videos and the methods without are trained only on simulation data.}
}
\begin{tabular}{lcc}
\toprule
Method & minADE\textsubscript{1}($\downarrow$)   & minFDE\textsubscript{1} ($\downarrow$)      \\ 
\midrule
Social-LSTM~\cite{alahi2016social}  & 23.10 & 44.27 \\
Social-GAN~\cite{gupta2018social}  & 30.42   & 60.70  \\ 
Next~\cite{liang2019peeking}  & 19.78 & 42.43\\
Multiverse~\cite{liang2020garden} & 18.51 & 35.84 \\
\midrule
Multiverse (Trained on Sim.)~\cite{liang2020garden} & 22.94 & 43.35 \\
SimAug & 21.73  & 42.22 \\
SimAug + finetune  & \textbf{17.96}  & \textbf{34.68} \\
\bottomrule
\end{tabular}
\label{table:actev}
\end{table}

==> tables/sdd.tex <==
\begin{table}[]
\centering
%\small
\caption{State-of-the-art comparison on the Stanford Drone Dataset (SDD). Numbers are minimal errors over 20 predictions and lower the better. Baseline numbers are taken from \cite{sadeghian2018sophie,deo2020trajectory}. ``SimAug'' is trained without using SDD training data and ``SimAug + finetune'' is further finetuned on SDD training data.}
\begin{tabular}{lcc}
\toprule
Method & minADE\textsubscript{20}($\downarrow$)   & minFDE\textsubscript{20} ($\downarrow$)      \\
\midrule
Social-LSTM~\cite{alahi2016social} & 31.19 & 56.97 \\
Social-GAN~\cite{gupta2018social} & 27.25   &  41.44 \\ 
DESIRE~\cite{lee2017desire} &  19.25 & 34.05 \\ 
SoPhie~\cite{sadeghian2018sophie} &  16.27 & 29.38 \\ 
Multiverse~\cite{liang2020garden} & 14.78 & 27.09 \\
IDL~\cite{li2019way} &  13.93 & 24.40 \\ 
P2T\textsubscript{IRL}~\cite{deo2020trajectory} &  12.58 & 22.07 \\ 
\midrule
SimAug & 12.03  & 23.98 \\
SimAug + finetune & \textbf{10.27}  & \textbf{19.71} \\
\bottomrule
\end{tabular}
\label{table:sdd}
\end{table}
